Noninvasive Anisotropic Identification of Magnetic Properties in Toroidal Shaped Magnetic Steel

This research proposes a model-free inverse approach for identifying the nonlinear anisotropic single-valued magnetic constitutive characteristics of soft magnetic materials from boundary measurements. Using the harmonic approximation, the internal magnetic flux density B and magnetic field strength H are independently reconstructed from the measured boundary data, thus avoiding the limitation of using a predefined parametric B--H mapping function. Subsequently, the reconstructed fields are spatially averaged along selected collection lines to recover the B--H characteristics of the principal directions. Numerical results demonstrate high reconstruction accuracy for unperturbed data and good robustness against Gaussian perturbations of the boundary measurements, with the overall mean error remaining below 5% for a 10% noise level. These results indicate that under the harmonic-field assumptions, the field-based reconstruction provides a simple and computationally efficient framework for non-invasive identification of nonlinear anisotropic magnetic constitutive characteristics.

==> sections/Assumptions.tex <==
\section{Forward Problem Formulation}
% \subsection{Two-Dimensional Magnetostatic Approximation and Symmetry Reduction}

\subsection{Forward Problem: Magnetostatic Model }

Under the magnetostatic assumption, the magnetic field in the two-dimensional domain is described by
\[
\mathbf{H} = \begin{bmatrix} H_x \\ H_y \end{bmatrix},
\quad
\mathbf{B} = \begin{bmatrix} B_x \\ B_y \end{bmatrix}.
\]
In the ferromagnetic core $\Omega_c$, the nonlinear anisotropic magnetic behavior is represented by the single-valued constitutive mapping

\begin{equation}
\mathbf{B} = \boldsymbol{\mathcal{B}}(\mathbf{H}) = \begin{bmatrix} \mathcal{B}_x(H_x) \\ \mathcal{B}_y(H_y) \end{bmatrix},
\quad
\text{in } \Omega_c.
\label{eq:BH-aniso}
\end{equation}
In the non-magnetic regions, the permeability is assumed to be equal to the vacuum permeability $\mu_0$, such that
\[
\mathbf{B} = \mu_0\mathbf{H},
\quad
\text{in } \Omega\setminus\overline{\Omega}_c.
\]
Hence, the constitutive relation over the entire computational domain can be written as
\[
\mathbf{B} = \begin{cases}
\boldsymbol{\mathcal{B}}(\mathbf{H}), & \text{in } \Omega_c, \\[2mm]
\mu_0\mathbf{H}, & \text{in } \Omega\setminus\overline{\Omega}_c.
\end{cases}
\]

The magnetostatic problem is governed by
\begin{equation}
\begin{cases}
\nabla\cdot\mathbf{B} = 0, & \text{in } \Omega, \\[1mm]
\nabla\times\mathbf{H} = \mathbf{J}, & \text{in } \Omega,
\end{cases}
\label{eq:govern_eqs}
\end{equation}
with
\[
\mathbf{J} =
\begin{cases}
\mathbf{J}_b,
& \text{in } \Omega_b,\\[1mm]
\mathbf{0},
& \text{in } \Omega_c,\\[1mm]
\mathbf{J}_o,
& \text{in } \Omega_o.
\end{cases}
\]


The problem is solved together with the above piecewise constitutive relation.
Introducing the two-dimensional magnetic vector potential through
\[
\mathbf{B} = \nabla\times(A\mathbf{e}_z),
\]
a homogeneous Dirichlet boundary condition is imposed on the external boundary,
\begin{equation}
    \label{eq:DC_Gamma}
A = 0,
\quad
\text{on } \Gamma.
\end{equation}

\subsection{Boundary Measurements and Cauchy Data}

The available magnetic measurements are assumed to collect the normal component of the magnetic flux density and the tangential component of the magnetic field strength on the interfaces. 
Assuming that no surface current is present at the material interfaces, the normal component of $\mathbf{B}$ and the tangential component of $\mathbf{H}$ are continuous across each interface. Hence, for \(i\in\{b,o\}\)
\[
\mathbf{n}_i\cdot\mathbf{B}^{+} = \mathbf{n}_i\cdot\mathbf{B}^{-} = B_{n,i},
\quad
\mathbf{t}_i\cdot\mathbf{H}^{+} = \mathbf{t}_i\cdot\mathbf{H}^{-} = H_{t,i},
\quad
\text{on } \Gamma_i .
\]
where $\mathbf{n}_i$ and $\mathbf{t}_i$ denote the unit normal and tangential vectors to $\Gamma_i$, respectively.

In this case, the available measurement data is the Cauchy data on the two interfaces, for $i\in\{b,o\}$, the Cauchy data is donated as:
\begin{equation}
\mathcal{C}
=
\left\{
\mathcal{C}_b,\,
\mathcal{C}_o
\right\},
\quad
\mathcal{C}_i
=
\left\{
B_{n,i},\,
H_{t,i}
\right\},
\quad \text{on } \Gamma_i.
\label{eq:Cauchy}
\end{equation}
In this simulations, the Cauchy data is collected by solving \eqref{eq:Cauchy} with homogenous Dirichlet boundary condition \eqref{eq:DC_Gamma}. The proposal of this research is to use the Cauchy data to construct the anisotropic single-valued magnetic constitutive relation.

\subsection{Inverse Problem Formulations}
\subsection{Harmonic Field Considerations}

==> sections/Feedbacks.tex <==
\section{Feedbacks from reviewer}

\subsection*{Reviewer: 1}

Comments to the Author
\begin{enumerate}
    \item The B-H curve of the identified magnetic sample should be supplemented in this work.
    \item Can this method consider the influence of the temperature?
    \item Can this approach be used to predicted the demagnetization curve of the magnetic sample?
\end{enumerate}

\subsection*{Reviewer: 2}

Comments to the Author
\begin{enumerate}
    \item A non-invasive method for identifying the unknown single-valued B-H curve of soft magnetic materials is proposed in this paper, which demonstrates certain novelty. It is suggested that further theoretical derivations be provided, and the applicability and limitations of the proposed method under complex hysteresis characteristics or strongly nonlinear conditions be discussed in more detail.
    \item The paper is currently mainly focused on theoretical analysis and illustrative results, while the experimental validation is relatively insufficient. It is suggested that additional validation using practical measurement data be included, and comparisons with traditional B-H curve measurement methods be provided.
\end{enumerate}


\subsection*{Reviewer: 3}

Comments to the Author
The research problem has practical engineering significance. To address the discrepancy between conventional material testing results and the actual performance of processed components, a reasonable research direction is proposed. By integrating the magnetic field inverse problem with the identification of nonlinear magnetic materials, the study demonstrates certain theoretical innovation. The proposed method is applicable to the acquisition of magnetic property parameters for electrical machine core materials.At present, the proposed approach remains more of a theoretical methodological framework, with insufficient experimental or practical validation.


\subsection*{Reza}

I read the paper; it is well written and easy to read. I have two minor comments:

- In sections III and IV, you are talking about measured data on Cauchy points, but later in section V, you use forward simulation results to identify the B-H characteristics. It would be nice to briefly elaborate on the possibility of measuring boundary values at Cauchy points. Otherwise, it is a bit difficult to see the value of the work without knowing the possibility of measuring boundary values in practice. This will also help the reader to better understand section V.B and the reason for the robustness analysis for the measurement noise.

- In Figure 3, I recommend you to replace the the actual BH curve with the average BH data obtained from the forward problem for different excitation currents, in a similar way that you have done it for the Inverse restotation. By making this change, the reader can better see the high accuracy in the inverse reconstruction.  
